First-Ever Deployment of a SiPM-on-Tile Calorimeter in a Collider: A Parasitic Test with 200 GeV $pp$ Collisions at RHIC

We describe the testing of a prototype SiPM-on-tile iron-scintillator calorimeter at the Relativistic Heavy Ion Collider (RHIC) during its 200 GeV $pp$ run in 2024. The prototype, measuring $20 \times 20 \, \text{cm}^{2}$ and 24 radiation lengths in depth, was positioned in the STAR experimental hall, approximately 8 m from the interaction point and 65 cm from the beam line, covering a pseudorapidity range of about $3.1<\eta<3.4$. By using the dark current of a reference SiPM as a radiation monitor, we estimate that the prototype was exposed to a fluence of about $10^{10}$ 1-MeV $n_{\mathrm{eq}}$/cm$^2$. Channel-by-channel calibration was performed in a data-driven way with the signature from minimum-ionizing particles during beam-on conditions. A Geant4 detector simulation, with inputs from the Pythia8 event generator, describes measurements of energy spectra and hit multiplicities reasonably well. These results mark the first deployment, commissioning, calibration, and long-term operation of a SiPM-on-tile calorimeter in a collider environment. This experimental campaign will guide detector designs and operational strategies for the ePIC detector at the future EIC, as well as other applications.

==> IntegratedRate.tex <==
\section{Trigger Logic and Integrated Rate}
\label{sec:dataset}
A scan of the trigger threshold was performed during beam-on conditions to study the trigger rate at different thresholds. The left panel of Figure~\ref{fig:statistics} shows how the trigger rate changed with the trigger tile threshold for independent trigger streams based on signals from a single tile. These streams used tiles 1, 2, and 3, referred to as T1, T2, and T3, which are positioned at the front or middle of the prototype (as described in Section~\ref{sec:setup}).

Various thresholds were tested throughout the commissioning process. Ultimately, the trigger thresholds for different trigger logic configurations were stabilized and set between 10 and 50 mV, resulting in rates ranging from a few Hz to several tens of Hz under optimized conditions.

The official RHIC 2024 run of 200 GeV $pp$ collisions took place from April through the end of September, followed by a two-week period of heavy-ion ($AuAu$) collisions in October. The commissioning period for our test, primarily focused on testing and debugging various aspects of the DAQ software, lasted until June 4th, as shown by the gap between the two red lines in the left panel of Figure~\ref{fig:statistics}. After commissioning, data collection proceeded smoothly, yielding over 100 million good events by the end of the run. During this time, 1219 runs were collected for $pp$ collisions and 125 for $AuAu$ collisions, which passed quality assurance based on metrics such as rate and average hit multiplicity.  

The events collected by this DAQ system include real $pp$ collisions, along with particles from other sources such as beam-gas and beam-halo interactions. In the absence of reference signals from other detectors or a reference clock from RHIC or STAR, the setup configuration and trigger strategy were unable to reject these background events.



